A data-centric approach to class-specific bias in image data augmentation

Data augmentation (DA) enhances model generalization in computer vision but may introduce biases, impacting class accuracy unevenly. Our study extends this inquiry, examining DA's class-specific bias across various datasets, including those distinct from ImageNet, through random cropping. We evaluated this phenomenon with ResNet50, EfficientNetV2S, and SWIN ViT, discovering that while residual models showed similar bias effects, Vision Transformers exhibited greater robustness or altered dynamics. This suggests a nuanced approach to model selection, emphasizing bias mitigation. We also refined a "data augmentation robustness scouting" method to manage DA-induced biases more efficiently, reducing computational demands significantly (training 112 models instead of 1860; a reduction of factor 16.2) while still capturing essential bias trends.

==> meta-data.tex <==
\def\thesistitle{A data-centric approach to class-specific bias in image data augmentation}
\def\shorttitle{} % Add these so that they show up on top of pages if needed.
\def\yourname{Athanasios Angelakis, Andrey Rass}
\def\shortname{} % Add these so that they show up on top of pages if needed.
\def\yourprogramme{}
% \def\yourcourse{Data Science in Action or Cognitive Science \& Artificial Intelligence}
\def\yourstudentnumber{} % legacy var so that formatter doesn't break
\def\finalmonth{} % legacy var so that formatter doesn't break
\def\finalyear{} % legacy var so that formatter doesn't break
\def\supervisor{} % legacy var so that formatter doesn't break
\def\committee{} % legacy var so that formatter doesn't break

\title{\thesistitle{}}

==> title0.tex <==
\title{\vspace{-1cm} % Adjust vertical space as needed
{\bf \Large A data-centric approach to class-specific bias in image data augmentation}
\rule{\textwidth}{2pt}
\rule{\textwidth}{3pt}}

\author{
\begin{tabular}{cc} 
\textbf{Athanasios Angelakis} & \textbf{Andrey Rass} \\
\textit{Amsterdam University Medical Center} & \textit{Den Haag, Netherlands} \\
\textit{University of Amsterdam - Data Science Center} & \textit{anvrass@gmail.com} \\
\textit{Amsterdam Public Health Research Institute} &  \\
\textit{Amsterdam, Netherlands} &  \\
\textit{a.angelakis@amsterdamumc.nl} & \\
\end{tabular}
}
\date{} % Empty date if you don't want it to show

